Unite and Conquer: Plug & Play Multi-Modal Synthesis using Diffusion Models

Generating photos satisfying multiple constraints find broad utility in the content creation industry. A key hurdle to accomplishing this task is the need for paired data consisting of all modalities (i.e., constraints) and their corresponding output. Moreover, existing methods need retraining using paired data across all modalities to introduce a new condition. This paper proposes a solution to this problem based on denoising diffusion probabilistic models (DDPMs). Our motivation for choosing diffusion models over other generative models comes from the flexible internal structure of diffusion models. Since each sampling step in the DDPM follows a Gaussian distribution, we show that there exists a closed-form solution for generating an image given various constraints. Our method can unite multiple diffusion models trained on multiple sub-tasks and conquer the combined task through our proposed sampling strategy. We also introduce a novel reliability parameter that allows using different off-the-shelf diffusion models trained across various datasets during sampling time alone to guide it to the desired outcome satisfying multiple constraints. We perform experiments on various standard multimodal tasks to demonstrate the effectiveness of our approach. More details can be found in https://nithin-gk.github.io/projectpages/Multidiff/index.html

==> metrics/alt_metrics.tex <==


\begin{table*}[!t]
\begin{center}
\setlength{\tabcolsep}{10pt}
\scalebox{0.8}{
\begin{tabular}{l l | c c c c c| c c c c c}
\toprule[0.15em]
%\rowcolor{color3} 
   && \multicolumn{5}{c|}{\textbf{CelebA dataset}} & \multicolumn{5}{c}{\textbf{FFHQ dataset}}  \\
\cline{2-12}
%\rowcolor{color3} 
   \textbf{Type}&\textbf{Method} & FID$\textcolor{black}{\downarrow}$ & LPIPS$\textcolor{black}{\downarrow}$& SSIM$\textcolor{black}{\uparrow}$ & mIoU$\textcolor{black}{\uparrow}$  & F1~$\textcolor{black}{\uparrow}$ &  FID$\textcolor{black}{\downarrow}$ & LPIPS$\textcolor{black}{\downarrow}$& SSIM$\textcolor{black}{\uparrow}$ & mIoU$\textcolor{black}{\uparrow}$  & F1~$\textcolor{black}{\uparrow}$   \\
\midrule[0.15em]
\multirow{5}{*}{Fine-Tuning} &SPADE\cite{park2019SPADE} &131.91 & 0.638 & 0.316 & 0.605&0.694 & 91.77& 0.624 & 0.340 & 0.649&0.728\\
&OASIS\cite{oasis}  & 118.67 & 0.624 & 0.318 & 0.579&0.663 & 99.94 &0.634 & 0.320 & 0.625&0.704 \\
&PIX2PIXHD\cite{wang2018pix2pixHD}& 153.19 & 0.611 & 0.282 & 0.716&0.819 & 223.85& 0.670 & 0.265 & 0.666&0.775  \\
&INADE\cite{tan2021diverse} &125.43& 0.632 & 0.279 & 0.881&0.932 & 134.11 & 0.656& 0.274 & 0.869&0.922 \\
% &DDPM\cite &111.35& 0.786 & 0.255 & 0.824&0.881 & 109.29& 0.703& 0.258 & 0.835&0.901 \\
\midrule[0.15em]
\multirow{5}{*}{Alternate} &SPADE\cite{park2019SPADE} & 89.29 & \textbf{0.523} & 0.376 & 0.890&0.936 & 75.73& \textbf{0.545} & 0.373 & 0.876&0.921\\
&OASIS\cite{oasis}  & 71.20 & 0.571 & 0.323 & 0.792&0.870 & 75.57 &0.593 & 0.331 & 0.786&0.863 \\
&PIX2PIXHD\cite{wang2018pix2pixHD}& 73.32 & 0.512 & 0.373 & 0.872&0.925 & 138.30& 0.560 & 0.363 & 0.840&0.898  \\
&INADE\cite{tan2021diverse} &54.27& 0.552  & 0.332& 0.887&0.933 & 47.40& 0.574 & 0.334  & 0.862&0.910\\
% &DDPM &55.23& 0.663  & 0.368&0.909&0.947 & 72.94& 0.681 & 0.365& 0.909&0.942  \\
\midrule[0.15em]
% \midrule[0.1em]


&TediGAN\cite{xia2021tedigan} &69.51 & 0.4823 & 0.417 & 0.834&0.905 & 125.27& 0.545 & 0.409&0.813 & 0.887\\
&OURS &\textbf{26.09} & 0.519 & \textbf{0.416} & \textbf{0.911}&\textbf{0.948} & \textbf{33.60}& 0.542 & \textbf{0.421}&\textbf{0.919} & \textbf{0.950} \\


\bottomrule[0.1em]
\end{tabular}}
\caption{Quantitative results for semantic labels to face generation on CelebA and FFHQ datasets. The alternate training based strategy and fine-tuning based training strategy are shown in the corresponding sections. $(\uparrow)$/  $(\downarrow)$ represents higher/ lower the metric lower the metrics, the better respectively. 
}
\label{table:semantic}
\end{center}
\vspace{-2em}
\end{table*}

==> suppl_tex/imgs_1.tex <==
\begin{figure}[tb!]
    \centering
    \setlength{\tabcolsep}{0.5pt}
    {\small
    \renewcommand{\arraystretch}{0.5} 
    \begin{tabular}{c c c c c c c c c c}
    \captionsetup{type=figure, font=scriptsize}
    \raisebox{0.1in}{\rotatebox{90}{\small \emph{$0.0$}
 }}
  \includegraphics[width=0.135\linewidth]{cvpr2023-author_kit-v1_1-1/bothsides/0.0_0.0_0.jpg}
  \includegraphics[width=0.135\linewidth]{cvpr2023-author_kit-v1_1-1/bothsides/0.0_0.2_0.jpg}
  \includegraphics[width=0.135\linewidth]{cvpr2023-author_kit-v1_1-1/bothsides/0.0_0.4_0.jpg}
  \includegraphics[width=0.135\linewidth]{cvpr2023-author_kit-v1_1-1/bothsides/0.0_0.5_0.jpg}
  \includegraphics[width=0.135\linewidth]{cvpr2023-author_kit-v1_1-1/bothsides/0.0_0.6_0.jpg}
  \includegraphics[width=0.135\linewidth]{cvpr2023-author_kit-v1_1-1/bothsides/0.0_0.8_0.jpg}
  \includegraphics[width=0.135\linewidth]{cvpr2023-author_kit-v1_1-1/bothsides/0.0_1.0_0.jpg}
 \tabularnewline
     \raisebox{0.1in}{\rotatebox{90}{\small \emph{$0.2$}
 }}
  \includegraphics[width=0.135\linewidth]{cvpr2023-author_kit-v1_1-1/bothsides/0.2_0.0_0.jpg}
  \includegraphics[width=0.135\linewidth]{cvpr2023-author_kit-v1_1-1/bothsides/0.2_0.2_0.jpg}
  \includegraphics[width=0.135\linewidth]{cvpr2023-author_kit-v1_1-1/bothsides/0.2_0.4_0.jpg}
  \includegraphics[width=0.135\linewidth]{cvpr2023-author_kit-v1_1-1/bothsides/0.2_0.5_0.jpg}
  \includegraphics[width=0.135\linewidth]{cvpr2023-author_kit-v1_1-1/bothsides/0.2_0.6_0.jpg}
  \includegraphics[width=0.135\linewidth]{cvpr2023-author_kit-v1_1-1/bothsides/0.2_0.8_0.jpg}
  \includegraphics[width=0.135\linewidth]{cvpr2023-author_kit-v1_1-1/bothsides/0.2_1.0_0.jpg}
\tabularnewline
    \raisebox{0.1in}{\rotatebox{90}{\small \emph{$0.4$}
 }}
  \includegraphics[width=0.135\linewidth]{cvpr2023-author_kit-v1_1-1/bothsides/0.4_0.0_0.jpg}
  \includegraphics[width=0.135\linewidth]{cvpr2023-author_kit-v1_1-1/bothsides/0.4_0.2_0.jpg}
  \includegraphics[width=0.135\linewidth]{cvpr2023-author_kit-v1_1-1/bothsides/0.4_0.4_0.jpg}
  \includegraphics[width=0.135\linewidth]{cvpr2023-author_kit-v1_1-1/bothsides/0.4_0.5_0.jpg}
  \includegraphics[width=0.135\linewidth]{cvpr2023-author_kit-v1_1-1/bothsides/0.4_0.6_0.jpg}
  \includegraphics[width=0.135\linewidth]{cvpr2023-author_kit-v1_1-1/bothsides/0.4_0.8_0.jpg}
  \includegraphics[width=0.135\linewidth]{cvpr2023-author_kit-v1_1-1/bothsides/0.4_1.0_0.jpg}
\tabularnewline
    \raisebox{0.1in}{\rotatebox{90}{\small \emph{$0.5$}
 }}
  \includegraphics[width=0.135\linewidth]{cvpr2023-author_kit-v1_1-1/bothsides/0.5_0.0_0.jpg}
  \includegraphics[width=0.135\linewidth]{cvpr2023-author_kit-v1_1-1/bothsides/0.5_0.2_0.jpg}
  \includegraphics[width=0.135\linewidth]{cvpr2023-author_kit-v1_1-1/bothsides/0.5_0.4_0.jpg}
  \includegraphics[width=0.135\linewidth]{cvpr2023-author_kit-v1_1-1/bothsides/0.5_0.5_0.jpg}
  \includegraphics[width=0.135\linewidth]{cvpr2023-author_kit-v1_1-1/bothsides/0.5_0.6_0.jpg}
  \includegraphics[width=0.135\linewidth]{cvpr2023-author_kit-v1_1-1/bothsides/0.5_0.8_0.jpg}
  \includegraphics[width=0.135\linewidth]{cvpr2023-author_kit-v1_1-1/bothsides/0.5_1.0_0.jpg}
\tabularnewline
    \raisebox{0.1in}{\rotatebox{90}{\small \emph{$0.6$}
 }}
  \includegraphics[width=0.135\linewidth]{cvpr2023-author_kit-v1_1-1/bothsides/0.6_0.0_0.jpg}
  \includegraphics[width=0.135\linewidth]{cvpr2023-author_kit-v1_1-1/bothsides/0.6_0.2_0.jpg}
  \includegraphics[width=0.135\linewidth]{cvpr2023-author_kit-v1_1-1/bothsides/0.6_0.4_0.jpg}
  \includegraphics[width=0.135\linewidth]{cvpr2023-author_kit-v1_1-1/bothsides/0.6_0.5_0.jpg}
  \includegraphics[width=0.135\linewidth]{cvpr2023-author_kit-v1_1-1/bothsides/0.6_0.6_0.jpg}
  \includegraphics[width=0.135\linewidth]{cvpr2023-author_kit-v1_1-1/bothsides/0.6_0.8_0.jpg}
  \includegraphics[width=0.135\linewidth]{cvpr2023-author_kit-v1_1-1/bothsides/0.6_1.0_0.jpg}
\tabularnewline
    \raisebox{0.1in}{\rotatebox{90}{\small \emph{$0.8$}
 }}
  \includegraphics[width=0.135\linewidth]{cvpr2023-author_kit-v1_1-1/bothsides/0.8_0.0_0.jpg}
  \includegraphics[width=0.135\linewidth]{cvpr2023-author_kit-v1_1-1/bothsides/0.8_0.2_0.jpg}
   \includegraphics[width=0.135\linewidth]{cvpr2023-author_kit-v1_1-1/bothsides/0.8_0.4_0.jpg}
  \includegraphics[width=0.135\linewidth]{cvpr2023-author_kit-v1_1-1/bothsides/0.8_0.5_0.jpg}
  \includegraphics[width=0.135\linewidth]{cvpr2023-author_kit-v1_1-1/bothsides/0.8_0.6_0.jpg}
  \includegraphics[width=0.135\linewidth]{cvpr2023-author_kit-v1_1-1/bothsides/0.8_0.8_0.jpg}
  \includegraphics[width=0.135\linewidth]{cvpr2023-author_kit-v1_1-1/bothsides/0.8_1.0_0.jpg}
\tabularnewline
    \raisebox{0.1in}{\rotatebox{90}{\small \emph{$1.0$}
 }}
  \includegraphics[width=0.135\linewidth]{cvpr2023-author_kit-v1_1-1/bothsides/1.0_0.0_0.jpg}
  \includegraphics[width=0.135\linewidth]{cvpr2023-author_kit-v1_1-1/bothsides/1.0_0.2_0.jpg}
   \includegraphics[width=0.135\linewidth]{cvpr2023-author_kit-v1_1-1/bothsides/1.0_0.4_0.jpg}
  \includegraphics[width=0.135\linewidth]{cvpr2023-author_kit-v1_1-1/bothsides/1.0_0.5_0.jpg}
  \includegraphics[width=0.135\linewidth]{cvpr2023-author_kit-v1_1-1/bothsides/1.0_0.6_0.jpg}
  \includegraphics[width=0.135\linewidth]{cvpr2023-author_kit-v1_1-1/bothsides/1.0_0.8_0.jpg}
  \includegraphics[width=0.135\linewidth]{cvpr2023-author_kit-v1_1-1/bothsides/1.0_1.0_0.jpg}
    \tabularnewline
        \raisebox{0.1in}{\rotatebox{90}{
 }}
 \hspace{0.5mm}
%     \begin{minipage}{0.135\linewidth}
% \end{minipage}
% \begin{minipage}{0.135\linewidth}
% (10,0)
%  \end{minipage}
% \begin{minipage}{0.135\linewidth}
% (8,2)
% \end{minipage}
% \begin{minipage}{0.135\linewidth}
% (6,4)
% \end{minipage}
% \begin{minipage}{0.135\linewidth}
% (5,5)
% \end{minipage}
% \begin{minipage}{0.135\linewidth}
% (4,6)
% \end{minipage}
% \begin{minipage}{0.135\linewidth}
% (2,8)
% \end{minipage}
% \begin{minipage}{0.135\linewidth}
% (0,10)
% \end{minipage}
    % \tabularnewline
   $\scriptsize{Text}\xrightarrow[\text{weighing factor}]{\hspace*{3cm}}\scriptsize{Class}$
  \tabularnewline
% {\small\hspace{15pt}Tibetan terrier\hskip10pt Teddy bear \hskip15pt Triceratops \hskip15pt Tree frog \hskip15pt Otterhound \hspace{20pt}Tibetan terrier\hskip10pt Teddy bear \hskip15pt Triceratops \hskip20pt Tree frog \hskip20pt Otterhound }\\
\vspace{2mm}
\vspace{-2\baselineskip}
\end{tabular}}
\vspace{-0.8cm}
\hspace{20pt}\captionof{figure}{\textbf{The role of reliability factor for multimodal generation.} Here, the vertical row going down denotes increasing reliability to the text model.}
\label{fig:glideablation1}
\vspace{-2mm}
\end{figure}%


==> tex_base_files/ablation_subfigure.tex <==
\begin{figure}[t!]
    \centering
    \begin{subfigure}[t]{0.134\linewidth}
      \captionsetup{justification=centering, labelformat=empty, font=scriptsize}
     \includegraphics[width=1\linewidth]{cvpr2023-author_kit-v1_1-1/bothsides/0.0_0.0_0.jpg}
    \includegraphics[width=1\linewidth]{cvpr2023-author_kit-v1_1-1/bothsides/0.2_0.0_0.jpg}
        \includegraphics[width=1\linewidth]{cvpr2023-author_kit-v1_1-1/bothsides/0.4_0.0_0.jpg}
            \includegraphics[width=1\linewidth]{cvpr2023-author_kit-v1_1-1/bothsides/0.5_0.0_0.jpg}
                \includegraphics[width=1\linewidth]{cvpr2023-author_kit-v1_1-1/bothsides/0.6_0.0_0.jpg}
                 \includegraphics[width=1\linewidth]{cvpr2023-author_kit-v1_1-1/bothsides/0.8_0.0_0.jpg}
             \includegraphics[width=1\linewidth]{cvpr2023-author_kit-v1_1-1/bothsides/1.0_0.0_0.jpg}                    
    \end{subfigure}
    \begin{subfigure}[t]{0.134\linewidth}
      \captionsetup{justification=centering, labelformat=empty, font=scriptsize}
     \includegraphics[width=1\linewidth]{cvpr2023-author_kit-v1_1-1/bothsides/0.0_0.2_0.jpg}
    \includegraphics[width=1\linewidth]{cvpr2023-author_kit-v1_1-1/bothsides/0.2_0.2_0.jpg}
        \includegraphics[width=1\linewidth]{cvpr2023-author_kit-v1_1-1/bothsides/0.4_0.2_0.jpg}
            \includegraphics[width=1\linewidth]{cvpr2023-author_kit-v1_1-1/bothsides/0.5_0.2_0.jpg}
                \includegraphics[width=1\linewidth]{cvpr2023-author_kit-v1_1-1/bothsides/0.6_0.2_0.jpg}
                 \includegraphics[width=1\linewidth]{cvpr2023-author_kit-v1_1-1/bothsides/0.8_0.2_0.jpg}
             \includegraphics[width=1\linewidth]{cvpr2023-author_kit-v1_1-1/bothsides/1.0_0.2_0.jpg}
    \end{subfigure}
    \begin{subfigure}[t]{0.134\linewidth}
      \captionsetup{justification=centering, labelformat=empty, font=scriptsize}
      \includegraphics[width=1\linewidth]{cvpr2023-author_kit-v1_1-1/bothsides/0.0_0.4_0.jpg}
    \includegraphics[width=1\linewidth]{cvpr2023-author_kit-v1_1-1/bothsides/0.2_0.4_0.jpg}
        \includegraphics[width=1\linewidth]{cvpr2023-author_kit-v1_1-1/bothsides/0.4_0.4_0.jpg}
            \includegraphics[width=1\linewidth]{cvpr2023-author_kit-v1_1-1/bothsides/0.5_0.4_0.jpg}
                \includegraphics[width=1\linewidth]{cvpr2023-author_kit-v1_1-1/bothsides/0.6_0.4_0.jpg}
                 \includegraphics[width=1\linewidth]{cvpr2023-author_kit-v1_1-1/bothsides/0.8_0.4_0.jpg}
             \includegraphics[width=1\linewidth]{cvpr2023-author_kit-v1_1-1/bothsides/1.0_0.4_0.jpg}
    \end{subfigure}
    \begin{subfigure}[t]{0.134\linewidth}
       \includegraphics[width=1\linewidth]{cvpr2023-author_kit-v1_1-1/bothsides/0.0_0.5_0.jpg}
    \includegraphics[width=1\linewidth]{cvpr2023-author_kit-v1_1-1/bothsides/0.2_0.5_0.jpg}
        \includegraphics[width=1\linewidth]{cvpr2023-author_kit-v1_1-1/bothsides/0.4_0.5_0.jpg}
            \includegraphics[width=1\linewidth]{cvpr2023-author_kit-v1_1-1/bothsides/0.5_0.5_0.jpg}
                \includegraphics[width=1\linewidth]{cvpr2023-author_kit-v1_1-1/bothsides/0.6_0.5_0.jpg}
                 \includegraphics[width=1\linewidth]{cvpr2023-author_kit-v1_1-1/bothsides/0.8_0.5_0.jpg}
             \includegraphics[width=1\linewidth]{cvpr2023-author_kit-v1_1-1/bothsides/1.0_0.5_0.jpg}
    \end{subfigure}
   \begin{subfigure}[t]{0.134\linewidth}
       \includegraphics[width=1\linewidth]{cvpr2023-author_kit-v1_1-1/bothsides/0.0_0.6_0.jpg}
    \includegraphics[width=1\linewidth]{cvpr2023-author_kit-v1_1-1/bothsides/0.2_0.6_0.jpg}
        \includegraphics[width=1\linewidth]{cvpr2023-author_kit-v1_1-1/bothsides/0.4_0.6_0.jpg}
            \includegraphics[width=1\linewidth]{cvpr2023-author_kit-v1_1-1/bothsides/0.5_0.6_0.jpg}
                \includegraphics[width=1\linewidth]{cvpr2023-author_kit-v1_1-1/bothsides/0.6_0.6_0.jpg}
                 \includegraphics[width=1\linewidth]{cvpr2023-author_kit-v1_1-1/bothsides/0.8_0.6_0.jpg}
             \includegraphics[width=1\linewidth]{cvpr2023-author_kit-v1_1-1/bothsides/1.0_0.6_0.jpg}
    \end{subfigure}
   \begin{subfigure}[t]{0.134\linewidth}
       \includegraphics[width=1\linewidth]{cvpr2023-author_kit-v1_1-1/bothsides/0.0_0.8_0.jpg}
    \includegraphics[width=1\linewidth]{cvpr2023-author_kit-v1_1-1/bothsides/0.2_0.8_0.jpg}
        \includegraphics[width=1\linewidth]{cvpr2023-author_kit-v1_1-1/bothsides/0.4_0.8_0.jpg}
            \includegraphics[width=1\linewidth]{cvpr2023-author_kit-v1_1-1/bothsides/0.5_0.8_0.jpg}
                \includegraphics[width=1\linewidth]{cvpr2023-author_kit-v1_1-1/bothsides/0.6_0.8_0.jpg}
                 \includegraphics[width=1\linewidth]{cvpr2023-author_kit-v1_1-1/bothsides/0.8_0.8_0.jpg}
             \includegraphics[width=1\linewidth]{cvpr2023-author_kit-v1_1-1/bothsides/1.0_0.8_0.jpg}
    \end{subfigure}
   \begin{subfigure}[t]{0.134\linewidth}
       \includegraphics[width=1\linewidth]{cvpr2023-author_kit-v1_1-1/bothsides/0.0_1.0_0.jpg}
    \includegraphics[width=1\linewidth]{cvpr2023-author_kit-v1_1-1/bothsides/0.2_1.0_0.jpg}
        \includegraphics[width=1\linewidth]{cvpr2023-author_kit-v1_1-1/bothsides/0.4_1.0_0.jpg}
            \includegraphics[width=1\linewidth]{cvpr2023-author_kit-v1_1-1/bothsides/0.5_1.0_0.jpg}
                \includegraphics[width=1\linewidth]{cvpr2023-author_kit-v1_1-1/bothsides/0.6_1.0_0.jpg}
                 \includegraphics[width=1\linewidth]{cvpr2023-author_kit-v1_1-1/bothsides/0.8_1.0_0.jpg}
             \includegraphics[width=1\linewidth]{cvpr2023-author_kit-v1_1-1/bothsides/1.0_1.0_0.jpg}
    \end{subfigure}
    
    \vspace{-3mm}    \caption{ $\scriptsize{Text}\xrightarrow[\text{weighing factor}]{\hspace*{2cm}}\scriptsize{Class}$ }
    \label{fig:glideablation1}
  \end{figure}


==> tex_base_files/blue_jay_comp.tex <==
\begin{figure*}[htb!]
    \centering
    \setlength{\tabcolsep}{0.5pt}
    {\small
    \renewcommand{\arraystretch}{0.5} 
    \begin{tabular}{c c c c c c c c c c c c}
    \captionsetup{type=figure, font=scriptsize}
 \includegraphics[width=0.06\linewidth]{cvpr2023-author_kit-v1_1-1/bluejay/normal/0_17.jpg}
 \includegraphics[width=0.06\linewidth]{cvpr2023-author_kit-v1_1-1/bluejay/normal/1_17.jpg}
 \includegraphics[width=0.06\linewidth]{cvpr2023-author_kit-v1_1-1/bluejay/normal/2_17.jpg}
 \includegraphics[width=0.06\linewidth]{cvpr2023-author_kit-v1_1-1/bluejay/normal/3_17.jpg}
  \includegraphics[width=0.06\linewidth]{cvpr2023-author_kit-v1_1-1/bluejay/normal/20_17.jpg}
    \hspace{1mm}
 \includegraphics[width=0.06\linewidth]{cvpr2023-author_kit-v1_1-1/bluejay/direc_guided/0_17.jpg}
 \includegraphics[width=0.06\linewidth]{cvpr2023-author_kit-v1_1-1/bluejay/direc_guided/1_17.jpg}
 \includegraphics[width=0.06\linewidth]{cvpr2023-author_kit-v1_1-1/bluejay/direc_guided/2_17.jpg}
 \includegraphics[width=0.06\linewidth]{cvpr2023-author_kit-v1_1-1/bluejay/direc_guided/3_17.jpg}
  \includegraphics[width=0.06\linewidth]{cvpr2023-author_kit-v1_1-1/bluejay/direc_guided/20_17.jpg}
  \hspace{1mm}
  
 \includegraphics[width=0.06\linewidth]{cvpr2023-author_kit-v1_1-1/bluejay/direc_rand/0_17.jpg}
 \includegraphics[width=0.06\linewidth]{cvpr2023-author_kit-v1_1-1/bluejay/direc_rand/1_17.jpg}
 \includegraphics[width=0.06\linewidth]{cvpr2023-author_kit-v1_1-1/bluejay/direc_rand/2_17.jpg}
 \includegraphics[width=0.06\linewidth]{cvpr2023-author_kit-v1_1-1/bluejay/direc_rand/3_17.jpg}
  \includegraphics[width=0.06\linewidth]{cvpr2023-author_kit-v1_1-1/bluejay/direc_rand/20_17.jpg}
 \tabularnewline
       \includegraphics[width=0.06\linewidth]{cvpr2023-author_kit-v1_1-1/bluejay/normal/4_17.jpg}
   \includegraphics[width=0.06\linewidth]{cvpr2023-author_kit-v1_1-1/bluejay/normal/5_17.jpg}
    \includegraphics[width=0.06\linewidth]{cvpr2023-author_kit-v1_1-1/bluejay/normal/6_17.jpg}
     \includegraphics[width=0.06\linewidth]{cvpr2023-author_kit-v1_1-1/bluejay/normal/7_17.jpg}
  \includegraphics[width=0.06\linewidth]{cvpr2023-author_kit-v1_1-1/bluejay/normal/21_17.jpg}
      \hspace{1mm}
      
    \includegraphics[width=0.06\linewidth]{cvpr2023-author_kit-v1_1-1/bluejay/direc_guided/4_17.jpg}
   \includegraphics[width=0.06\linewidth]{cvpr2023-author_kit-v1_1-1/bluejay/direc_guided/5_17.jpg}
    \includegraphics[width=0.06\linewidth]{cvpr2023-author_kit-v1_1-1/bluejay/direc_guided/6_17.jpg}
     \includegraphics[width=0.06\linewidth]{cvpr2023-author_kit-v1_1-1/bluejay/direc_guided/7_17.jpg}
     \includegraphics[width=0.06\linewidth]{cvpr2023-author_kit-v1_1-1/bluejay/direc_guided/21_17.jpg}
     \hspace{1mm}
   
  \includegraphics[width=0.06\linewidth]{cvpr2023-author_kit-v1_1-1/bluejay/direc_rand/4_17.jpg}
   \includegraphics[width=0.06\linewidth]{cvpr2023-author_kit-v1_1-1/bluejay/direc_rand/5_17.jpg}
    \includegraphics[width=0.06\linewidth]{cvpr2023-author_kit-v1_1-1/bluejay/direc_rand/6_17.jpg}
     \includegraphics[width=0.06\linewidth]{cvpr2023-author_kit-v1_1-1/bluejay/direc_rand/7_17.jpg}
     \includegraphics[width=0.06\linewidth]{cvpr2023-author_kit-v1_1-1/bluejay/direc_guided/21_17.jpg}
 
 \tabularnewline    
     
        \includegraphics[width=0.06\linewidth]{cvpr2023-author_kit-v1_1-1/bluejay/normal/8_17.jpg}
       \includegraphics[width=0.06\linewidth]{cvpr2023-author_kit-v1_1-1/bluejay/normal/9_17.jpg}
        \includegraphics[width=0.06\linewidth]{cvpr2023-author_kit-v1_1-1/bluejay/normal/10_17.jpg}
         \includegraphics[width=0.06\linewidth]{cvpr2023-author_kit-v1_1-1/bluejay/normal/11_17.jpg}
            \includegraphics[width=0.06\linewidth]{cvpr2023-author_kit-v1_1-1/bluejay/normal/22_17.jpg}      
         \hspace{1mm}

      \includegraphics[width=0.06\linewidth]{cvpr2023-author_kit-v1_1-1/bluejay/direc_guided/8_17.jpg}
       \includegraphics[width=0.06\linewidth]{cvpr2023-author_kit-v1_1-1/bluejay/direc_guided/9_17.jpg}
        \includegraphics[width=0.06\linewidth]{cvpr2023-author_kit-v1_1-1/bluejay/direc_guided/10_17.jpg}
         \includegraphics[width=0.06\linewidth]{cvpr2023-author_kit-v1_1-1/bluejay/direc_guided/11_17.jpg}
            \includegraphics[width=0.06\linewidth]{cvpr2023-author_kit-v1_1-1/bluejay/direc_guided/22_17.jpg}  
        \hspace{1mm}
           \includegraphics[width=0.06\linewidth]{cvpr2023-author_kit-v1_1-1/bluejay/direc_rand/8_17.jpg}
       \includegraphics[width=0.06\linewidth]{cvpr2023-author_kit-v1_1-1/bluejay/direc_rand/9_17.jpg}
        \includegraphics[width=0.06\linewidth]{cvpr2023-author_kit-v1_1-1/bluejay/direc_rand/10_17.jpg}
         \includegraphics[width=0.06\linewidth]{cvpr2023-author_kit-v1_1-1/bluejay/direc_rand/11_17.jpg}
         \includegraphics[width=0.06\linewidth]{cvpr2023-author_kit-v1_1-1/bluejay/direc_rand/22_17.jpg}
    \tabularnewline
          \includegraphics[width=0.06\linewidth]{cvpr2023-author_kit-v1_1-1/bluejay/normal/12_17.jpg}
           \includegraphics[width=0.06\linewidth]{cvpr2023-author_kit-v1_1-1/bluejay/normal/13_17.jpg}
            \includegraphics[width=0.06\linewidth]{cvpr2023-author_kit-v1_1-1/bluejay/normal/14_17.jpg}
              \includegraphics[width=0.06\linewidth]{cvpr2023-author_kit-v1_1-1/bluejay/normal/15_17.jpg}
              \includegraphics[width=0.06\linewidth]{cvpr2023-author_kit-v1_1-1/bluejay/normal/23_17.jpg}
\hspace{1mm}
          \includegraphics[width=0.06\linewidth]{cvpr2023-author_kit-v1_1-1/bluejay/direc_guided/12_17.jpg}
           \includegraphics[width=0.06\linewidth]{cvpr2023-author_kit-v1_1-1/bluejay/direc_guided/13_17.jpg}
            \includegraphics[width=0.06\linewidth]{cvpr2023-author_kit-v1_1-1/bluejay/direc_guided/14_17.jpg}
              \includegraphics[width=0.06\linewidth]{cvpr2023-author_kit-v1_1-1/bluejay/direc_guided/15_17.jpg}
              \includegraphics[width=0.06\linewidth]{cvpr2023-author_kit-v1_1-1/bluejay/direc_guided/23_17.jpg}

\hspace{1mm}
          \includegraphics[width=0.06\linewidth]{cvpr2023-author_kit-v1_1-1/bluejay/direc_rand/12_17.jpg}
           \includegraphics[width=0.06\linewidth]{cvpr2023-author_kit-v1_1-1/bluejay/direc_rand/13_17.jpg}
            \includegraphics[width=0.06\linewidth]{cvpr2023-author_kit-v1_1-1/bluejay/direc_rand/14_17.jpg}
              \includegraphics[width=0.06\linewidth]{cvpr2023-author_kit-v1_1-1/bluejay/direc_rand/15_17.jpg}
                 \includegraphics[width=0.06\linewidth]{cvpr2023-author_kit-v1_1-1/bluejay/direc_rand/23_17.jpg}           
\tabularnewline
     \includegraphics[width=0.06\linewidth]{cvpr2023-author_kit-v1_1-1/bluejay/normal/16_17.jpg}
   \includegraphics[width=0.06\linewidth]{cvpr2023-author_kit-v1_1-1/bluejay/normal/17_17.jpg}
    \includegraphics[width=0.06\linewidth]{cvpr2023-author_kit-v1_1-1/bluejay/normal/18_17.jpg}
     \includegraphics[width=0.06\linewidth]{cvpr2023-author_kit-v1_1-1/bluejay/normal/19_17.jpg}
     \includegraphics[width=0.06\linewidth]{cvpr2023-author_kit-v1_1-1/bluejay/normal/24_17.jpg}
      \hspace{1mm}
      
     \includegraphics[width=0.06\linewidth]{cvpr2023-author_kit-v1_1-1/bluejay/direc_guided/16_17.jpg}
   \includegraphics[width=0.06\linewidth]{cvpr2023-author_kit-v1_1-1/bluejay/direc_guided/17_17.jpg}
    \includegraphics[width=0.06\linewidth]{cvpr2023-author_kit-v1_1-1/bluejay/direc_guided/18_17.jpg}
     \includegraphics[width=0.06\linewidth]{cvpr2023-author_kit-v1_1-1/bluejay/direc_guided/19_17.jpg}
     \includegraphics[width=0.06\linewidth]{cvpr2023-author_kit-v1_1-1/bluejay/direc_guided/24_17.jpg}
     \hspace{1mm}
   
  \includegraphics[width=0.06\linewidth]{cvpr2023-author_kit-v1_1-1/bluejay/direc_rand/4_17.jpg}
   \includegraphics[width=0.06\linewidth]{cvpr2023-author_kit-v1_1-1/bluejay/direc_rand/5_17.jpg}
    \includegraphics[width=0.06\linewidth]{cvpr2023-author_kit-v1_1-1/bluejay/direc_rand/6_17.jpg}
     \includegraphics[width=0.06\linewidth]{cvpr2023-author_kit-v1_1-1/bluejay/direc_rand/7_17.jpg}
     \includegraphics[width=0.06\linewidth]{cvpr2023-author_kit-v1_1-1/bluejay/direc_rand/24_17.jpg} 
% {\scriptsize\hspace{15pt}Tibetan terrier\hskip10pt Teddy bear \hskip15pt Triceratops \hskip15pt Tree frog \hskip15pt Otterhound \hspace{20pt}Tibetan terrier\hskip10pt Teddy bear \hskip15pt Triceratops \hskip20pt Tree frog \hskip20pt Otterhound }\\
\tabularnewline

\begin{minipage}{0.33\linewidth}
\hspace{2cm}
Direct Sampling
\end{minipage}
\begin{minipage}{0.33\linewidth}
\hspace{1.5cm}
Classifier-free guidance\cite{ho2020denoising}
\end{minipage}
\begin{minipage}{0.33\linewidth}
\hspace{1.5cm}
Random Conditioning
\end{minipage}
\end{tabular}}
\vspace{-0.4cm}
\hspace{20pt}\captionof{figure}{A visual comparison illustrating the effect of using a randomly sampled class instaead of null conditioning on ImageNet conditional generation model. Random sampling isable to achieve almost the same performance as classifier free guidance}
\label{fig:bluejaypic}
\vspace{-2mm}
\end{figure*}%


==> tex_base_files/semantic_sppl_obo.tex <==
\begin{figure*}[t!]
    \centering
    \begin{subfigure}[t]{0.137\linewidth}
      \captionsetup{justification=centering, labelformat=empty, font=scriptsize}
    %   \includegraphics[width=1\linewidth]{cvpr2023-author_kit-v1_1-1/semantic_synth/newlabels/00035.jpg}
     \includegraphics[width=1\linewidth]{cvpr2023-author_kit-v1_1-1/semantic_synth/One_by_One/celeba/input_new/10.jpg}
       \includegraphics[width=1\linewidth]{cvpr2023-author_kit-v1_1-1/semantic_synth/One_by_One/celeba/input_new/1035.jpg}
    \includegraphics[width=1\linewidth]{cvpr2023-author_kit-v1_1-1/semantic_synth/One_by_One/celeba/input_new/113.jpg}
     \includegraphics[width=1\linewidth]{cvpr2023-author_kit-v1_1-1/semantic_synth/One_by_One/celeba/input_new/116.jpg} 
        \includegraphics[width=1\linewidth]{cvpr2023-author_kit-v1_1-1/semantic_synth/One_by_One/ffhq/input_new/00035.jpg}
     \includegraphics[width=1\linewidth]{cvpr2023-author_kit-v1_1-1/semantic_synth/One_by_One/ffhq/input_new/00065.jpg}
      \includegraphics[width=1\linewidth]{cvpr2023-author_kit-v1_1-1/semantic_synth/One_by_One/ffhq/input_new/00067.jpg}
       \includegraphics[width=1\linewidth]{cvpr2023-author_kit-v1_1-1/semantic_synth/One_by_One/ffhq/input_new/00092.jpg}
      \caption{Semantic label}
    \end{subfigure}
       \begin{subfigure}[t]{0.137\linewidth}
      \captionsetup{justification=centering, labelformat=empty, font=scriptsize}
  
     \includegraphics[width=1\linewidth]{cvpr2023-author_kit-v1_1-1/semantic_synth/One_by_One/celeba/oasis/10.jpg}
       \includegraphics[width=1\linewidth]{cvpr2023-author_kit-v1_1-1/semantic_synth/One_by_One/celeba/oasis/1035.jpg}
    \includegraphics[width=1\linewidth]{cvpr2023-author_kit-v1_1-1/semantic_synth/One_by_One/celeba/oasis/113.jpg}
     \includegraphics[width=1\linewidth]{cvpr2023-author_kit-v1_1-1/semantic_synth/One_by_One/celeba/oasis/116.jpg} 
        \includegraphics[width=1\linewidth]{cvpr2023-author_kit-v1_1-1/semantic_synth/One_by_One/ffhq/oasis/00035.jpg}
     \includegraphics[width=1\linewidth]{cvpr2023-author_kit-v1_1-1/semantic_synth/One_by_One/ffhq/oasis/00065.jpg}
      \includegraphics[width=1\linewidth]{cvpr2023-author_kit-v1_1-1/semantic_synth/One_by_One/ffhq/oasis/00067.jpg}
       \includegraphics[width=1\linewidth]{cvpr2023-author_kit-v1_1-1/semantic_synth/One_by_One/ffhq/oasis/00092.jpg}
      \caption{SPADE\cite{park2019SPADE}}
    \end{subfigure}
    \begin{subfigure}[t]{0.137\linewidth}
      \captionsetup{justification=centering, labelformat=empty, font=scriptsize}
  
     \includegraphics[width=1\linewidth]{cvpr2023-author_kit-v1_1-1/semantic_synth/One_by_One/celeba/spade/10.jpg}
       \includegraphics[width=1\linewidth]{cvpr2023-author_kit-v1_1-1/semantic_synth/One_by_One/celeba/spade/1035.jpg}
    \includegraphics[width=1\linewidth]{cvpr2023-author_kit-v1_1-1/semantic_synth/One_by_One/celeba/spade/113.jpg}
     \includegraphics[width=1\linewidth]{cvpr2023-author_kit-v1_1-1/semantic_synth/One_by_One/celeba/spade/116.jpg} 
        \includegraphics[width=1\linewidth]{cvpr2023-author_kit-v1_1-1/semantic_synth/One_by_One/ffhq/spade/00035.jpg}
     \includegraphics[width=1\linewidth]{cvpr2023-author_kit-v1_1-1/semantic_synth/One_by_One/ffhq/spade/00065.jpg}
      \includegraphics[width=1\linewidth]{cvpr2023-author_kit-v1_1-1/semantic_synth/One_by_One/ffhq/spade/00067.jpg}
       \includegraphics[width=1\linewidth]{cvpr2023-author_kit-v1_1-1/semantic_synth/One_by_One/ffhq/spade/00092.jpg}
      \caption{SPADE\cite{park2019SPADE}}
    \end{subfigure}
    \begin{subfigure}[t]{0.137\linewidth}
      \captionsetup{justification=centering, labelformat=empty, font=scriptsize}
    \includegraphics[width=1\linewidth]{cvpr2023-author_kit-v1_1-1/semantic_synth/One_by_One/celeba/pix2pixhd/10.jpg}
       \includegraphics[width=1\linewidth]{cvpr2023-author_kit-v1_1-1/semantic_synth/One_by_One/celeba/pix2pixhd/1035.jpg}
    \includegraphics[width=1\linewidth]{cvpr2023-author_kit-v1_1-1/semantic_synth/One_by_One/celeba/pix2pixhd/113.jpg}
     \includegraphics[width=1\linewidth]{cvpr2023-author_kit-v1_1-1/semantic_synth/One_by_One/celeba/pix2pixhd/116.jpg} 
        \includegraphics[width=1\linewidth]{cvpr2023-author_kit-v1_1-1/semantic_synth/One_by_One/ffhq/pix2pixhd/00035.jpg}
     \includegraphics[width=1\linewidth]{cvpr2023-author_kit-v1_1-1/semantic_synth/One_by_One/ffhq/pix2pixhd/00065.jpg}
      \includegraphics[width=1\linewidth]{cvpr2023-author_kit-v1_1-1/semantic_synth/One_by_One/ffhq/pix2pixhd/00067.jpg}
       \includegraphics[width=1\linewidth]{cvpr2023-author_kit-v1_1-1/semantic_synth/One_by_One/ffhq/pix2pixhd/00092.jpg}
      \caption{PIX2PIXHD\cite{wang2018pix2pixHD}}
    \end{subfigure}
    \begin{subfigure}[t]{0.137\linewidth}
      \captionsetup{justification=centering, labelformat=empty, font=scriptsize}
  \includegraphics[width=1\linewidth]{cvpr2023-author_kit-v1_1-1/semantic_synth/One_by_One/celeba/spade/10.jpg}
       \includegraphics[width=1\linewidth]{cvpr2023-author_kit-v1_1-1/semantic_synth/One_by_One/celeba/inade/1035.jpg}
    \includegraphics[width=1\linewidth]{cvpr2023-author_kit-v1_1-1/semantic_synth/One_by_One/celeba/inade/113.jpg}
     \includegraphics[width=1\linewidth]{cvpr2023-author_kit-v1_1-1/semantic_synth/One_by_One/celeba/inade/116.jpg} 
        \includegraphics[width=1\linewidth]{cvpr2023-author_kit-v1_1-1/semantic_synth/One_by_One/ffhq/inade/00035.jpg}
     \includegraphics[width=1\linewidth]{cvpr2023-author_kit-v1_1-1/semantic_synth/One_by_One/ffhq/inade/00065.jpg}
      \includegraphics[width=1\linewidth]{cvpr2023-author_kit-v1_1-1/semantic_synth/One_by_One/ffhq/inade/00067.jpg}
       \includegraphics[width=1\linewidth]{cvpr2023-author_kit-v1_1-1/semantic_synth/One_by_One/ffhq/inade/00092.jpg}
      \caption{INADE\cite{tan2021diverse}}
    \end{subfigure}
    \begin{subfigure}[t]{0.137\linewidth}
      \captionsetup{justification=centering, labelformat=empty, font=scriptsize}
    \includegraphics[width=1\linewidth]{cvpr2023-author_kit-v1_1-1/semantic_synth/One_by_One/celeba/ddpm/10.jpg}
       \includegraphics[width=1\linewidth]{cvpr2023-author_kit-v1_1-1/semantic_synth/One_by_One/celeba/ddpm/1035.jpg}
    \includegraphics[width=1\linewidth]{cvpr2023-author_kit-v1_1-1/semantic_synth/One_by_One/celeba/ddpm/113.jpg}
     \includegraphics[width=1\linewidth]{cvpr2023-author_kit-v1_1-1/semantic_synth/One_by_One/celeba/ddpm/116.jpg} 
        \includegraphics[width=1\linewidth]{cvpr2023-author_kit-v1_1-1/semantic_synth/One_by_One/ffhq/ddpm/00035.jpg}
     \includegraphics[width=1\linewidth]{cvpr2023-author_kit-v1_1-1/semantic_synth/One_by_One/ffhq/ddpm/00065.jpg}
      \includegraphics[width=1\linewidth]{cvpr2023-author_kit-v1_1-1/semantic_synth/One_by_One/ffhq/ddpm/00067.jpg}
       \includegraphics[width=1\linewidth]{cvpr2023-author_kit-v1_1-1/semantic_synth/One_by_One/ffhq/ddpm/00092.jpg}
      \caption{DDPM\cite{ho2020denoising}}
    \end{subfigure}
    \begin{subfigure}[t]{0.137\linewidth}
      \captionsetup{justification=centering, labelformat=empty, font=scriptsize}
 \includegraphics[width=1\linewidth]{cvpr2023-author_kit-v1_1-1/semantic_synth/One_by_One/celeba/our/10.jpg}
       \includegraphics[width=1\linewidth]{cvpr2023-author_kit-v1_1-1/semantic_synth/One_by_One/celeba/our/1035.jpg}
    \includegraphics[width=1\linewidth]{cvpr2023-author_kit-v1_1-1/semantic_synth/One_by_One/celeba/our/113.jpg}
     \includegraphics[width=1\linewidth]{cvpr2023-author_kit-v1_1-1/semantic_synth/One_by_One/celeba/our/116.jpg} 
        \includegraphics[width=1\linewidth]{cvpr2023-author_kit-v1_1-1/semantic_synth/One_by_One/ffhq/our/00035.jpg}
     \includegraphics[width=1\linewidth]{cvpr2023-author_kit-v1_1-1/semantic_synth/One_by_One/ffhq/our/00065.jpg}
      \includegraphics[width=1\linewidth]{cvpr2023-author_kit-v1_1-1/semantic_synth/One_by_One/ffhq/our/00067.jpg}
       \includegraphics[width=1\linewidth]{cvpr2023-author_kit-v1_1-1/semantic_synth/One_by_One/ffhq/our/00092.jpg}
      \caption{OURS}
    \end{subfigure}
    \vspace{-3mm}    \caption{\textbf{Qualitative comparisons for semantic to face generation.} In this case, a single model is trained by first trainign over face then finetuning for hair for all comparison methods. During Inference time all the modalities are taken from a single dataset and the proposed sampling technique is used.}
    \label{fig:facesematicsupp}
  \end{figure*}

